Concept-Aware Denoising Graph Neural Network for Micro-Video Recommendation

Recently, micro-video sharing platforms such as Kuaishou and Tiktok have become a major source of information for people's lives. Thanks to the large traffic volume, short video lifespan and streaming fashion of these services, it has become more and more pressing to improve the existing recommender systems to accommodate these challenges in a cost-effective way. In this paper, we propose a novel concept-aware denoising graph neural network (named CONDE) for micro-video recommendation. CONDE consists of a three-phase graph convolution process to derive user and micro-video representations: warm-up propagation, graph denoising and preference refinement. A heterogeneous tripartite graph is constructed by connecting user nodes with video nodes, and video nodes with associated concept nodes, extracted from captions and comments of the videos. To address the noisy information in the graph, we introduce a user-oriented graph denoising phase to extract a subgraph which can better reflect the user's preference. Despite the main focus of micro-video recommendation in this paper, we also show that our method can be generalized to other types of tasks. Therefore, we also conduct empirical studies on a well-known public E-commerce dataset. The experimental results suggest that the proposed CONDE achieves significantly better recommendation performance than the existing state-of-the-art solutions.

==> untitled <==
\section{Related Work}
\subsection{micro-video recommendation}
Different from item contents in e-commerce sites, micro-videos teem with distinctive characteristics. MMGCN\cite{mmgcn} incorporates multi-modal information into a collaborative filtering framework. It capture modal-specific user preferences by separately constructing a user-item bipartite graph for each modality. ALPINE\cite{ALPINE/MM2019}also designs a graph-based sequential network for recommendation task, which can better model users' diverse and dynamic interest. THACIL\cite{THACIL/MM2018} propose hierarchical attention mechanism for user' short-term and long-term behavior modeling.

\subsection{Graph Embedding}
Graph embedding learning aims to learn low-dimensional vectorized embedding of nodes or edges from the graph topology structures. Some shallow graph embedding methods, including
\cite{deepwalk/KDD2014,line/www15,node2vec/KDD16,metapath2vec/KDD2017}, learn the node representations (embedding vectors) in an unsupervised way, then the node representations can be fed into the downstream graph mining tasks for further training. This process is similar to pre-training in NLP. 
\subsection{GNN}
Recent years have witnessed the 
superior performance of graph neural networks in graph analytics and network embedding tasks. In practice, GNN methods are more expressive than traditional feature-based methods.
The key idea of GNN is to recursively aggregate information and messages from local neighborhoods. Graph convolution network\cite{GCN/iclr201} is the first work that introduces the convolution operation to graph, which gathers the one-hop neighbors' information of source nodes via aggregate operations and achieve message passing by stacking multiple GCN layers. Graph attention network\cite{GAT/iclr2018} introduces the attention mechanism into GNNs, which enables the model to learn the importance of different neighbor nodes, and aggregates information of the whole neighborhood with attention weights. \\
However, the advances and applications of GNNs are largely designed for homogeneous graphs in which all nodes or links are of the same type. 
To deal with heterogeneous graph that contains different types of nodes and links, HAN\cite{HAN/www2019} modify original GAT model with a semantic attention layer to learn the importance of different metapaths. 

\subsection{Graph-based Recommendation}
In recent years, recommender systems has become increasingly important in online services, such as Amazon, YouTube, Netflix, Spotify, LinkedIn, Facebook, IMDb, etc. Many conpanies are now making great efforts to develop and deploy recommender systems, by which they can catch users' interests more accurately, and help users quickly get what they want, thus providing better service to users and making more profits. \\
Recommender systems build heterogeneous graphs based on historical interactions and side infomation, where the nodes can be users, items, entities in knowledge graph (side infomation), and the edges can be different types of interactions like click, purchase, add to cart, or relation of co-occurance. Taking heterogeneous nature of graphs into consideration, \cite{hahe,MAGNN,MEIRec,GATNE,HetGNN} extend the recommennation framework to more complex heterogeneous networks based on metapaths.
AGNN\cite{qian2019solving} designs an attribute graph based on user-item interactions and utilizes VAE to learn the distribution of attributes for cold-start users/items.
Pinsage\cite{pinSage/KDD18} combines random wallks and graph convolution layers to aggregate and propagate neiborhood inforamations. Similarly, GraphSAGE\cite{graphSage/nips17} extends the original graph convolution style framework to the inductive setting, which is able to deal with new user and new items. And it is able to handle the large scale graph with batch training and neighborhood sampling. 
MG-BERT\cite{MG-BERT} apply the bert model on item homogeneous graph to pretrain the item representation, including graph structure reconstruction and masked node feature reconstruction.\\
Many researchers regard Knowledge Graphs as complementary tools of great help. With its rich semantic information, knowledge graphs can explore potential connection between users and items, therefore making recommendation more accurate and explainable. 
RippleNet\cite{ripplenet} is a path-based method that first assigns entities in the KG with initial embeddings and then samples ripple sets from the KG based on user's historically clicking items. It uses attention networks to simulate user preferences on sampled ripple sets to represents a user. Then, the user’s representation is combined with item’s representation to predict the CTR of this user-item pair. Some of its extensions\cite{KGAT/KDD2019,akge,KNI/KDD2019} focus on using the embedding propagation mechanism on the item Knowledge Graph. 
DKN\cite{dkn} is another representative work that incorporates knowledge graph representation into news recommendation.
\subsection{Graph Denoising}
Graph denoising and sparsification is a promising solution to address the “noisy” graph challenge by prune away task-irrelevant edges, like \cite{PTDnet/WSDM2019} . And \cite{robust/ICML2019} learns robust representation and improve the generalization performance of GNNs through reinforcement learning. 

